Targeted Intervention in Random Graphs

We consider a setting where individuals interact in a network, each choosing actions which optimize utility as a function of neighbors' actions. A central authority aiming to maximize social welfare at equilibrium can intervene by paying some cost to shift individual incentives, and the optimal intervention can be computed using the spectral decomposition of the graph, yet this is infeasible in practice if the adjacency matrix is unknown. In this paper, we study the question of designing intervention strategies for graphs where the adjacency matrix is unknown and is drawn from some distribution. For several commonly studied random graph models, we show that there is a single intervention, proportional to the first eigenvector of the expected adjacency matrix, which is near-optimal for almost all generated graphs when the budget is sufficiently large. We also provide several efficient sampling-based approaches for approximately recovering the first eigenvector when we do not know the distribution. On the whole, our analysis compares three categories of interventions: those which use no data about the network, those which use some data (such as distributional knowledge or queries to the graph), and those which are fully optimal. We evaluate these intervention strategies on synthetic and real-world network data, and our results suggest that analysis of random graph models can be useful for determining when certain heuristics may perform well in practice.

==> conclusion.tex <==
\iffalse

\section{Conclusion}
\label{conclusion}



\section{Future Work}

%There is still work to be done on the power law result. We are working in the $G(w)$ model, but a challenge is that the result we would like to use about the mixing time of random walks only holds in the fixed degree sequence model (to our knowledge). It is also possible that power law graphs are disconnected when generated according to the $G(w)$ problem, and disconnected graphs are outside of the scope of t 

The $G(w)$ model captures a wide variety of interesting graphs, but some of interest are not handled at present by our results. In particular, power law graphs generated according to the model are not guaranteed to be connected with high probability. Another generating model, where exact degrees are fixed, is connected with high probability and also is known to have a mixing time of $O(\log n)$. However, edges are not sampled independently, and different techniques would be needed to bound the deviation of the first eigenvector from its expectation.

We believe it may be possible to extend results to stochastic block model graphs, where interventions would only need to know the block membership of each vertex (as well as block size and relative in-group and out-group connectivity). More generally, our approach shows that the problem of computing a near-optimal intervention in a random graph can be reduced to approximating the expected first eigenvector of the graph within a small norm bound, provided that the random model satisfies the ``large enough eigenvalues'' and ``non-vanishing spectral gap'' properties.

We also conjecture that for any graph, the uniform intervention beats any random intervention from a distribution where all permutations have equal probability, i.e.\ adding randomness to an anonymous intervention never helps.

Another question of interest would be to explore tradeoffs between utility and inequality, measured in terms of the Gini coefficient of the utility distribution. In the large budget case, the utility of an agent will be a monotone function of their eigenvector centrality. In the case of $G(n,p)$ networks, this indicates that all agents will have similar utility under the optimal intervention. This is not the case in power law graphs, where the central agents will be better off. Here, a goal would be to obtain Pareto-optimal tradeoffs between the two objectives for a given budget.
\fi


==> oldtext.tex <==

\section{Experiments}
We construct a Python implementation of the Galeotti et al.\ model which enables the creation of random networks, parameter assignment, computation of Nash equilibria, and computation of social welfare. Our implementation additionally allows us to evaluate the impacts to social for any intervention in comparison with the dominant component of the optimal intervention. In addition to the optimal intervention, we propose five heuristic approaches, requiring varying degrees of information about the network structure.
\subsection{Proposed Heuristics}
We let $N$ denote the number of agents in the network. Most of these heuristic methods are parameterized by a value $K$, which indicates the number of agents whose utility functions are modified by the intervention. Presented below are descriptions for each of the interventions:
\begin{itemize}
    \item \textbf{Uniform:} The $b_i$ values for all agents are increased by $\sqrt{C/N}$, as this results in a total intervention cost of $C$.
    \item \textbf{Random-$K$:} The $b_i$ values for $K$ agents, selected randomly without replacement, are increased by $\sqrt{C/K}$.
    \item \textbf{Friends-$K$:} In this heuristic, we aim to select agents with high network centrality without knowledge of the edges in the graph. We choose $K$ agents by selecting an agent at random, including a random \textit{neighbor} of that agent in our set, and repeat until $K$ distinct agents have been selected. This biases our sample towards agents with high degree, as they are more likely to be the neighbor of a randomly selected vertex. The $b_i$ values for these $K$ agents are increased by $\sqrt{C/K}$.
    \item \textbf{Top-$K$:} The $b_i$ values for the $K$ agents with the most neighbors are increased by $\sqrt{C/K}$.
    \item \textbf{PageRank-$K$:} The $b_i$ values for the $K$ agents with the largest PageRank values are increased by $\sqrt{C/K}$.
\end{itemize}
For comparison, we also consider the limiting case of the optimal intervention as well as a baseline where no intervention is applied:
\begin{itemize}
    \item \textbf{OPT:} The $b_i$ values for all agents are increased in proportion with the dominant eigenvector of $G$ ($\sqrt{C}\mathbf{u}_1$).
    \item \textbf{Baseline:} All $b_i$ values are unchanged.
\end{itemize}

\subsection{Results}
For all experiments and for specification of parameter values for $C$ and $K$, we run multiple trials, randomizing over the construction of the network, the selection of targeted agents by our heuristics, and the distributions for agents' $b_i$ values. We fix the size of the network at 100 and include every edge with a 10\% probability. The value for $\beta$ is fixed at 0.1. Edges between agents $i$ and $j$ are represented by setting $g_{ij} = 1$; all values in the adjacency matrix corresponding to non-existent edges are set to 0.

\begin{figure}[H]
    \centering
    \includegraphics[width=8cm]{normal_dist_weights_2_05}
    \caption{Utility vs $K$ ($N=100$, $C=100$, 10\% connectivity, $\beta = 0.1$, $b_i \sim N(2,0.5)$)}
    \label{fig3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=8cm]{budget_k_20_normal_2_05}
    \caption{Utility vs $C$ ($N=100$, $K=20$, 10\% connectivity, $\beta = 0.1$, $b_i \sim N(2,0.5)$)}
    \label{fig4}
\end{figure}

\section{Efficacy Lower Bounds for Heuristic Interventions}
We consider a uniform intervention to be one applying an equal weight adjustment to all agents. In experimental results, this performed nearly as well as the optimal intervention, and we aim to develop theory which justifies this.


\subsection{Bounding the Largest Eigenvalue of Random Graphs}

\begin{theorem}[Erdos-Renyi Graphs \cite{krivelevich_sudakov_2003}]
Let $G= G(n,p)$ be a random graph with maximum degree $\delta$. Almost surely, $$\lambda_1(G) = (1+ o(1))\max(\sqrt{\delta}, np)$$
where $o(1)$ tends to 0 as $\max(\sqrt{\delta}, np)$ tends to infinity.
\end{theorem}

\begin{theorem}[Power Law Graphs Graphs \cite{Chung2003}]
Let $G$ be a random graph where the number of vertices with degree $k$ is proportional to $k^{-\beta}$. If $\beta > 2.5$, almost surely, $$\lambda_1(G) = (1+ o(1))\max(\sqrt{\delta})$$
where $\delta$ is the maximum degree in $G$ (for sufficiently large $\delta$).
\end{theorem}


\subsection{Decomposition of Improvements}
\textbf{Uniform: $\Delta b_i = \sqrt{C/N}$}\\
\textbf{OPT (limit): $\Delta b_i = \sqrt{C}\mathbf{u}_{1,i}$}\\
\begin{align*}
    a + \Delta a =&\; M^{-1} (b + \Delta b) \\ 
    =&\; M^{-1}b + M^{-1} \Delta b \\
    =&\; a + M^{-1} \Delta b \\
    \Delta a =&\;  M^{-1} \Delta b \\
    \Delta a_{U} =&\; M^{-1} \times (\sqrt{C/N} \cdot \mathbf{1})\\
    \Delta a_{OPT} =&\; M^{-1} \times \sqrt{C}\mathbf{u}_{1,i}\\
\end{align*} 
What can we say about the above in terms of the spectral properties of $G$? Given that, what can we say about the difference between the resulting changes in welfare?
\begin{align*}
    W_0 =&\; \langle b, a \rangle - 1/2 \langle a, a \rangle + \beta a' G a \\
    W_1 =&\;   \langle b + \Delta b, a + \Delta a \rangle - 1/2 \langle a + \Delta a, a + \Delta a \rangle + \beta (a + \Delta a)' G (a + \Delta a) \\
    =&\; \langle b, a \rangle + \langle \Delta b, a \rangle  + \langle b, \Delta a \rangle + \langle \Delta b, \Delta a \rangle \\ &- 1/2 (\langle a, a \rangle + 2 \langle a, \Delta a \rangle + \langle \Delta a, \Delta a \rangle )\\&+ \beta \langle a'G + \Delta a'G,  a+ \Delta a\rangle\\
    \Delta W =&\; \langle \Delta b, a \rangle + \langle b,  \Delta a \rangle + \langle\Delta b, \Delta a \rangle \\ &- \langle a, \Delta a \rangle - \frac{1}{2}\langle \Delta a, \Delta a \rangle \\ &+ \beta(a'G\Delta a + \Delta a'G a + \Delta a' G \Delta a) \\
     =&\; \langle \Delta b, M^{-1}b \rangle + \langle b,  \Delta a \rangle + \langle\Delta b, \Delta a \rangle \\ &- \langle M^{-1}b , \Delta a \rangle - \frac{1}{2}\langle \Delta a, \Delta a \rangle \\ &+ \beta((M^{-1}b )'G\Delta a + \Delta a'G (M^{-1}b ) + \Delta a' G \Delta a) \\
    =&\; \langle \Delta b, M^{-1}b \rangle + \langle b,  M^{-1} \Delta b \rangle + \langle\Delta b, M^{-1} \Delta b \rangle \\ &- \langle M^{-1}b , M^{-1} \Delta b \rangle - \frac{1}{2}\langle M^{-1} \Delta b, M^{-1} \Delta b \rangle \\ &+ \beta((M^{-1}b )'G(M^{-1} \Delta b) +  (M^{-1} \Delta b)'G (M^{-1}b ) +(M^{-1} \Delta b)' G (M^{-1} \Delta b)) \\
     =&\; \langle \Delta b, M^{-1}(b +\Delta b) \rangle + \langle (b - M^{-1}b  - \frac{1}{2} M^{-1} \Delta b) ,  M^{-1} \Delta b \rangle \\  &+ \beta((M^{-1}b )'G(M^{-1} \Delta b) +  (M^{-1} \Delta b)'G (M^{-1}(b + \Delta b)) \\
      =&\; \langle \Delta b + \beta ((M^{-1} \Delta b)'G)', M^{-1}(b +\Delta b) \rangle + \langle (b - M^{-1}b  - \frac{1}{2} M^{-1} \Delta b + (\beta(M^{-1}b )'G)' ,  M^{-1} \Delta b \rangle \\
\end{align*}

This gives us a closed form expression for change in welfare as a function of the graph parameters and the applied intervention -- there might be a better way to simplify this.

\begin{conjecture}[Lower Bound for Uniform Intervention Efficacy]
There is a function $f(b, \beta, G)$ such that:
\begin{align*}
    \lim_{C \rightarrow \infty}\frac{\Delta W_{OPT}(b, \beta, G)}{\Delta W_{U}(b, \beta, G)} \leq&\; f(b, \beta, G)
\end{align*}
Further, for some parameter regimes, $f$ is bounded by 1 + $o(1)$, where $o(1)$ tends to 0 as the size of $G$ grows.
\end{conjecture}

\noindent\emph{Proof idea}: For sufficiently large random $d$-regular graphs, the largest eigenvalue should tend towards a uniform vector. Further, the largest eigenvalue of a random $d$-regular graph is approximately $d$ (can't find a great reference but mentioned here: \href{http://www.mit.edu/~18.338/2012s/projects/yz_slides.pdf}{Eigenvalues of Random Graphs}). If $p > \frac{1}{\sqrt{n}}$ for a power law or Erdos-Renyi graph, the above theorems suggest that the graph's largest eigenvector is bounded by $np = \Tilde{d}$. This would show a convergence of the largest eigenvalues for a random regular graph and other suitable random graphs as $n\rightarrow \infty$ (with $p$ and $d$ parameterized by $n$); further, it may be possible to argue that the limit of the first eigenvector is near-uniform for certain graph distributions (this would imply our conjecture fairly directly). For example, it shouldn't be hard to argue (if not already proved) that large Erdos-Renyi graphs are approximately regular, i.e. a vanishing fraction of vertices have degree outside $[(1-\epsilon)np, (1+\epsilon)np]$ for any $\epsilon$. 

Another approach requiring fewer distributional assumptions would be to use the largest eigenvalue of $G$ to somehow quantify the norm of $\Delta a$ under the optimal intervention, although this may require some careful analysis of $M^{-1}$. We would then need to relate the change in actions to change in welfare, and show that the ratio of changes is decaying to 1 (or at least bounded by some constant factor not much larger than 1). 

This convergence should occur faster for larger $b$ and smaller $\beta$ values, as the optimal intervention is uniform when $\beta = 0$; it is unclear what the importance of the distribution of values in $b$ should be. 

This is discussed further in Section 6.


\section{Possible Desired Results}
\begin{itemize}
    \item Give a closed-form expression for change in welfare in terms of the intervention vector and network parameters
    \item As the budget and network size go to infinity, for ER graphs with $p$ large enough to satisfy Theorem 3 conditions, ratio of welfare increase for optimum and uniform interventions goes to zero.
    \begin{itemize}
        \item Idea: viewing the problem as optimization over a convex set, we can show that the expression for $\Delta W$ in terms of $\Delta b$ is locally Lipschitz in terms of other parameters and apply Theorem 3 to bound the loss in utility (requires that gap between centrality vectors vanishes faster than Lipschitz factor grows).
    \end{itemize}
    \item For ER graphs, can we show a ``PTAS''-style result for finite $n$?
    \item For power law graphs, can we show a constant approximation factor for the optimality of a top-$k$ degree intervention? (Do we take $k$ to maximize cosine similarity with the expected centrality vector?)
    \begin{itemize}
        \item Compute eigenvector of edge probability matrix
        \item Use Theorem 3 to show a bound on difference between expected and realized first eigenvector
        \item Show a constant bound on cosine similarity (or norm of difference?) with the top-$k$ intervention, for a suitably chosen $k$
    \end{itemize}
    \item Could we develop a distribution-free theorem that relates the (cosine) similarity of an intervention to the optimal intervention with its efficacy?
    \item We can convert any lower bound on the approximate optimality of an intervention to a budget scaling factor sufficient to equalize the cahnge in welfare
\end{itemize}

Links:
\begin{itemize}
    \item \href{https://arxiv.org/pdf/1709.10402.pdf}{Dasaratha}
    \item \href{https://www.combinatorics.org/ojs/index.php/eljc/article/view/v18i1p215/pdf}{Chung 11}
    \item \href{http://people.math.sc.edu/lu/papers/eigen.pdf}{Chung 03}
\end{itemize}








Proof sketch:
\begin{itemize}
    \item For a sufficiently large budget, the optimal intervention for the strategic complements case is almost entirely dominated by the first eigenvector (from \cite{Galeotti2017TargetingII})
    \item For a sufficiently large and dense power graph, the first eigenvector is close (both in norm and cosine similarity) to its expectation, which is well-characterized (and proportional to degree) 
    \item We can approximate the first eigenvector by selecting nodes via short random walks (need to read up on this more). 
    \item Q: how well can we approximate with $o(n)$ samples? What's the dependency on the power law parameter?
    \item Can estimate centralities of agents to arbitrary precision with infinite sampling, can probably get ``reasonable'' approximation with few samples (because most of the mass is concentrated on a small number of vertices, which can be found quickly with random walks)
    \item From Dasaratha 19 (page 17), need the degree of every vertex to grow with the size of the graph (ideally linearly) to get a good rate of convergence, this should be OK
    \item By the same Lipschitz argument as before, vanishing error of the estimator implies competitive ratio going to 1. 
\end{itemize}
Extensions:
\begin{itemize}
    \item If we don't know the power law parameter, can we estimate with samples? 
\end{itemize}


\begin{fact}The distribution of a random walk from an arbitrary start on a power law graph is within total variation distance $O(\frac{1}{\text{poly}(n)})$ from its stationary distribution after $O(\log n)$ steps.  
\end{fact}


\begin{fact}
    If a power law graph has a constant minimum degree $d_{\min}$, the sum of all degrees is $O(n)$.
\end{fact}
\begin{lemma}
    Let $\pi$ be the stationary distribution of a random walk on a power law graph $G$. We can compute an estimate of this distribution $\hat{\pi}$, such that $\norm{\pi - \hat{\pi}} \leq \epsilon$ with probability $1 - \delta$, using a random walk of length $O(\frac{n}{\epsilon^2} \log(n)\log(\frac{n}{\delta}))$.  \label{lemma:power-law-random-walk}
\end{lemma}
\begin{proof}
    Ignoring variation distance issue for now. Assume we can draw $m$ independent samples from the stationary distribution. Fix some vertex $i$. Let $X_j$ be the Bernoulli variable takinvalue 1 if the $j$th trial results in $i$ being sampled, and let $X = \sum_{j} X_j$. By the above facts, there is some constant $c$ such that all vertices have probability at least $\frac{c}{n}$ in the stationary distribution. Let $\mu = \E[X]$, which is at least $\frac{cm}{n}$ for all vertices. By a Chernoff-Hoeffding bound:
\begin{align*}
    \Pr[X \leq (1-\epsilon)\mu] \leq e^{-\epsilon^2 \mu / 2},
\end{align*}
and
\begin{align*}
    \Pr[X \geq (1+\epsilon)\mu] \leq e^{-\epsilon^2 \mu / 3}.
\end{align*}
Setting $e^{-\epsilon^2 \mu / 3} \leq \frac{\delta}{2n}$, taking the log of both sides, and multiplying by $-1$, we have that:
\begin{align*}
    \frac{\epsilon^2 \mu}{3} \geq \log \frac{2n}{\delta}
\end{align*}
and so taking $m \geq \frac{3n}{c\epsilon^2} \log( \frac{2n}{\delta})$ gives us a probability below $\frac{\delta}{2n}$ for each of the above events occurring. Union-bounding over all $2n$ events (2 per vertex) gives us a total failure probability below $\delta$.

Let $\hat{\pi}$ be the empirical distribution observed. Let $\pi_{\max}$ be the entrywise maximum of $\hat{\pi}$ and $\pi$ (which will have norm greater than 1).    

Each term is non-negative and the vector has norm 1. Because each entry is within a $(1 + \epsilon)$ factor of its value in $\pi$, the norm of the difference of the vectors is bounded by $\epsilon$ (this should be fleshed out a bit, maybe ends up being $2\epsilon$. could also just directly bound cosine similarity above $1 - \epsilon$).

\end{proof}

If we only care about a larger approximation ratio and need sublinear time, then it suffices to repeat the above analysis, but only capturing vertices with degree $O(n^{\gamma})$, where $0 < \gamma < 1$, which covers roughly $O(n^{1-\gamma})$ vertices. The remaining vertices will have degree between a constant and $O(n^{\gamma})$, and will constitute a constant fraction of the stationary distribution. We then apply a uniform intervention across the ``less prominent'' vertices, and the maximum degree ratio amongst this set is the bottleneck for our approximation ratio.  

I think it's also worth seeing how well a totally random intervention does (what's the expected cosine similarity between a fixed vector and a random vector?). My intuition is that a random vector is likely to be mostly orthogonal to a fixed vector in high dimensions, so could be quite bad for some graphs, but maybe less so for power law graphs. If the linear time intervention does substantially better than a random or uniform intervention, that's a good motivation to consider it as well. 

\subsection{Transform from Stationary Distribution to Eigenvector
  Centrality}


\subsection{Efficient Approximate Convergence}
Can we bound the number of updates required before all agents are playing $\epsilon$-best responses?

